DBGDGM: Dynamic Brain Graph Deep Generative Model

Graphs are a natural representation of brain activity derived from functional magnetic imaging (fMRI) data. It is well known that clusters of anatomical brain regions, known as functional connectivity networks (FCNs), encode temporal relationships which can serve as useful biomarkers for understanding brain function and dysfunction. Previous works, however, ignore the temporal dynamics of the brain and focus on static graphs. In this paper, we propose a dynamic brain graph deep generative model (DBGDGM) which simultaneously clusters brain regions into temporally evolving communities and learns dynamic unsupervised node embeddings. Specifically, DBGDGM represents brain graph nodes as embeddings sampled from a distribution over communities that evolve over time. We parameterise this community distribution using neural networks that learn from subject and node embeddings as well as past community assignments. Experiments demonstrate DBGDGM outperforms baselines in graph generation, dynamic link prediction, and is comparable for graph classification. Finally, an analysis of the learnt community distributions reveals overlap with known FCNs reported in neuroscience literature.

==> 3-related_work.tex <==
\section{Related work}
\label{related_work}

\paragraph{Dynamic graph generative models} Classic generative models for graph-structured data are designed for capturing a small set of specific properties (e.g., degree distribution, eigenvalues, modularity) of static graphs~\citep{erdos1960evolution, barabasi1999emergence, nowicki2001estimation}. DGMs that exploit the learning capacity of NNs are able to learn more expressive graph distributions~\citep{mehta2019stochastic, kipf2016variational, sarkar2020graph}. Recent DGMs for dynamic graphs are majority VAE-based~\citep{kingma2013auto} and cannot learn community representations~\citep{hajiramezanali2019variational, gracious2021neural, zhang2021disentangled}. The few that do, are designed for static graphs~\cite{sun2019vgraph, khan2021unsupervised, cavallari2017learning}. 

\paragraph{Learning representations of dynamic brain graphs} Unsupervised representation learning methods for DBGs tend to focus on clustering DBGs into a finite number of connectivity patterns that recur over time~\citep{allen2014tracking, spencer2022using}. Community detection is another commonly used method but mainly applied to static brain graphs~\citep{pavlovic2020multi, esfahlani2021modularity}. Extensions to DBGs are typically not end-to-end trainable and do not scale to multi-subject datasets~\citep{ting2020detecting, martinet2020robust}. Recent deep learning-based methods are predominately GNN-based~\citep{kim2021learning, dahan2021improving}. Unlike \model, these methods are supervised and focus on learning deterministic node- and graph-level representations.



%The application of DGMs to DBGs derived from real-world fMRI data remains under explored.



%\begin{figure}[!htbp]
%\centering
%\includegraphics[draft=false, width=0.8\textwidth]{figures/plate_diagram.pdf}
%\caption{Graphical model representation of \model. Latent and observed variables are represented by white-and gray-shaded circles, respectively. Solid black squares denote non-linear mappings parameterized by neural networks.}
%\label{fig:model}
%\end{figure}


% To date, there exits no benchmark for learning dynamic brain graph representation, either supervised or unsupervised for dynamic link prediction.

% ~\citep{kazemi2020representation, gupta2022survey}

% are the Erd{\H{o}}s-R{\'e}nyi model~\cite{erdos1960evolution} and the stochastic block model (SBM)~\cite{nowicki2001estimation}. Although originally formulated for static graphs, both families of model have been extended to include temporal dynamics~\cite{mandjes2019dynamic, xu2014dynamic}. SBMs are commonly applied to dynamic brain graphs due to their ability to simultaneously learn community structures~\citep{}


%xu2015stochastic xing2010state.

% More recent generative models for dynamic graphs include DYMOND~\cite{zeno2021dymond} and TagGen~\cite{}

% framework~\cite{guo2020systematic, faez2021deep}. In particular, ....



% Further related work on deep generative models for static and dynamic graphs can be found in the surveys of \cite{faez2021deep, guo2020systematic} and \cite{gupta2022survey}, respectively

% Many methods dynamic graph models \cite{zhang2017random}

% \subsection{Dynamic graph community detection}

% ComE algorithm [Cavallari et al., 2017] achieved state-of-the-art performances in detecting communities
% on graphs. The main idea of this algorithm is to alternate between embedding and learning communities by means of
% Gaussian mixture models.

% Community detection for graphs has been extensively studied~\cite{}. The majority of methods are algorithmic vs generative models.

% A classical approach to detect communities is spectral clustering

% generative models for community detection specify a generation process for graphs and cast community detection as an inference problem~\cite{}.

% The majority of works doing community detection on fMRI data use either MM or SBMs on static brain graphs~\cite{}.

% Applications of extensions of MM and SBMs to dynamic brain graphs derived from fMRI is limited since 

% DynGEM~\cite{goyal2018dyngem} uses a deep autoencoder framework to learn node embeddings from dynamic graphs. However, Unlike \model which uses a RNN to explicitly model temporal dependencies between embeddings at different timepoints, DynGEM has to reinitialize the parameters of the autoencoder at each timepoint with the parameters learnt at the previous timepoint.


% - Dynamic
% deep learning dynamic community detection
% Dynamic Community Detection via Adversarial Temporal Graph Representation Learning
%The majority of existing methods for community detection operate on static graphs \cite{Pavlovic2020}. On the other hand, methods for dynamic graphs either optimise a subjective measure of community quality \cite{Martinet2020} or assume nodes can only belong to a single community at a time \citep{Ting2020}. Further, the majority of graph convolutional approaches are supervised



%%%
% https://www.biorxiv.org/content/10.1101/2021.07.08.451590v1.full
% clustering algorithms such as K- means clustering (Damaraju, et al., 2014) (Allen, et al., 2014), hidden Markov models (HMM) (Vidaurre, Smith, & Woolrich, 2017), temporal ICA (TICA) (Yaesoubi, Miller, & Calhoun, 2015) allows to identify clustering-derived recurring connectivity patterns or dFC states.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Community detection
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Matrix factorization
%     - Chimera
%         - https://arxiv.org/pdf/1807.06560v1.pdf?ref=https://githubhelp.com
%         - https://github.com/renatolfc/chimera-stf/blob/master/chimera/chimera.py
        
% - ComE
%     - https://dl.acm.org/doi/pdf/10.1145/3132847.3132925
%     - https://github.com/andompesta/ComE
    
% GCN
%  -  MRFasGCN
%     - https://www.ijcai.org/Proceedings/2020/0486.pdf
    
    
% Survey on community detection
%     - https://arxiv.org/pdf/1608.00163.pdf
    
% dynnode2vec
%     - https://github.com/dmcbffeng/dynnode2vec_for_HiC


% http://www.cs.columbia.edu/~blei/seminar/2020-representation/readings/BengioCourvilleVincent2013a.pdf

% Among the various ways of learning representations, this paper
% focuses on deep learning methods: those that are formed by
% the composition of multiple non-linear transformations, with
% the goal of yielding more abstract – and ultimately more useful
% – representations. 
